Explainability of Highly Associated Fuzzy Churn Patterns in Binary Classification

Customer churn, particularly in the telecommunications sector, influences both costs and profits. As the explainability of models becomes increasingly important, this study emphasizes not only the explainability of customer churn through machine learning models, but also the importance of identifying multivariate patterns and setting soft bounds for intuitive interpretation. The main objective is to use a machine learning model and fuzzy-set theory with top-\textit{k} HUIM to identify highly associated patterns of customer churn with intuitive identification, referred to as Highly Associated Fuzzy Churn Patterns (HAFCP). Moreover, this method aids in uncovering association rules among multiple features across low, medium, and high distributions. Such discoveries are instrumental in enhancing the explainability of findings. Experiments show that when the top-5 HAFCPs are included in five datasets, a mixture of performance results is observed, with some showing notable improvements. It becomes clear that high importance features enhance explanatory power through their distribution and patterns associated with other features. As a result, the study introduces an innovative approach that improves the explainability and effectiveness of customer churn prediction models.

==> backup/backup.tex <==
\begin{table}[ht]
    \centering
    \caption{Comparison of performance metrics with adding top 1-5 highly associated fuzzy churn patterns using Table. \ref{tab:highutilityitemsets_withmaxcar} dataset 1}
    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
        \textbf{Metrics} & \textbf{Baseline} & \textbf{Top 1} & \textbf{Top 2} & \textbf{Top 3} & \textbf{Top 4} & \textbf{Top 5} \\
    \hline
        
        Accuracy & 95.7\% & \textbf{0.1\%} & \textbf{0.1\%} & \textbf{0.3\%} & \textbf{0.1\%} & 0.0\% \\
        Recall Rate & 76.2\% & 0.0\% & 0.0\% & \textbf{3.0\%} & \textbf{1.0\%} & \textbf{1.0\%} \\
        Precision & 93.9\% & \textbf{1.2\%} & \textbf{1.2\%} & -0.9\% & 0.0\% & -1.1\% \\
        F1 score & 84.2\% & \textbf{0.5\%} & \textbf{0.5\%} & \textbf{1.4\%} & \textbf{0.6\%} & \textbf{0.2\%} \\%    
        \hline
    \end{tabular}
    \label{tab:model performance enhancement_dataset1}
\end{table}

\begin{table}[ht]
    \centering
    \caption{Comparison of performance metrics with adding top 1-5 highly associated fuzzy churn patterns using Table. \ref{tab:highutilityitemsets_withmaxcar} dataset 2}
    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
        \textbf{Metrics} & \textbf{Baseline} & \textbf{Rank 1} & \textbf{Rank 2} & \textbf{Rank 3} & \textbf{Rank 4} & \textbf{Rank 5} \\
    \hline
        AUC & 90.6\% & 0.0\% & 0.0\% & 0.0\% & \textbf{0.4\%} & -0.1\% \\
        Accuracy & 95.6\% & 0.0\% & 0.0\% & \textbf{0.2\%} & 0.0\% & \textbf{0.2\%} \\
        Recall Rate & 92.1\% & 0.0\% & -1.5\% & -0.4\% & -1.0\% & \textbf{0.6\%} \\
        Precision & 77.9\% & 0.0\% & \textbf{1.5\%} & \textbf{1.5\%} & \textbf{1.0\%} & \textbf{0.5\%} \\
        F1 score & 84.4\% & 0.0\% & \textbf{0.3\%} & \textbf{0.7\%} & \textbf{0.2\%} & \textbf{0.6\%} \\
    \hline
    \end{tabular}
    \label{tab:model_performance_enhancement_dataset2}
\end{table}







 \begin{table}[!ht]
    \centering
    \caption{Attributes Overview for Dataset 3}
    \label{tab:attributes_overview3}
    \begin{tabular}{|l|l|}
        \hline
        \multicolumn{1}{|c|}{\textbf{Attribute}} & \multicolumn{1}{c|}{\textbf{Explanation}} \\
        \hline
        \textit{Anonymous Customer ID} & Distinct identity code for each customer \\
        \textit{Call Failures} & Count of unsuccessful call attempts \\
        \textit{Complains} & Binary indicator (0: No complains, 1: has complained) \\
        \textit{Subscription Length} & Duration of subscription in months \\
        \textit{Charge Amount} & Ranked attribute (0: minimal charge, 9: maximal charge) \\
        \textit{Seconds of Use} & Aggregate duration of call usage in seconds \\
        \textit{Frequency of Use} & Aggregate count of call instances \\
        \textit{Frequency of SMS} & Total count of SMS sent \\
        \textit{Distinct Called Numbers} & Count of unique phone numbers called \\
        \textit{Age Group} & Ranked attribute (1: younger demographic, 5: older demographic) \\
        \textit{Tariff Plan} & Binary (1: Pay-per-use, 2: contract-based) \\
        \textit{Status} & Binary (1: currently active, 2: not active) \\
        \textit{Churn} & Binary (1: has churned, 0: has not churned) - Target variable \\
        \textit{Customer Value} & Estimated value rating for the customer \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[!ht]
\centering
\caption{Variable Descriptions for Datasets}
\tiny
\label{tab:variable_descriptions}
\begin{tabular}{|l|p{10cm}|}
\hline
\textbf{Attribute} & \textbf{Explanation} \\
\hline
customer & Customer ID \\
calibrat & Calibration sample - 1; Validation sample - 0; \\
churn & Churn between 31-60 days after observation (missing for validation sample) \\
churndep & Churn (missing for validation sample) \\
revenue & Mean monthly revenue \\
mou & Mean monthly minutes of use \\
recchrge & Mean total recurring charge \\
directas & Mean number of director assisted calls \\
overage & Mean overage minutes of use \\
roam & Mean number of roaming calls \\
changem & \% Change in minutes of use \\
changer & \% Change in revenues \\
dropvce & Mean number of dropped voice calls \\
blckvce & Mean number of blocked voice calls \\
unansvce & Mean number of unanswered voice calls \\
custcare & Mean number of customer care calls \\
threeway & Mean number of three-way calls \\
mourec & Mean unrounded minutes of use received voice calls \\
outcalls & Mean number of outbound voice calls \\
incalls & Mean number of inbound voice calls \\
peakvce & Mean number of in and out peak voice calls \\
opeakvce & Mean number of in and out off-peak voice calls \\
dropblk & Mean number of dropped or blocked calls \\
callfwdv & Mean number of call forwarding calls \\
callwait & Mean number of call waiting calls \\
months & Months in Service \\
uniqsubs & Number of Unique Subs \\
actvsubs & Number of Active Subs \\
phones & \# Handsets Issued \\
models & \# Models Issued \\
eqpdays & Number of days of the current equipment \\
age1 & Age of first HH member \\
age2 & Age of second HH member \\
children & Presence of children in HH \\
credita & Highest credit rating - a \\
creditaa & High credit rating - aa \\
prizmrur & Prizm code is rural \\
prizmub & Prizm code is suburban \\
prizmtwn & Prizm code is town \\
refurb & Handset is refurbished \\
webcap & Handset is web capable \\
truck & Subscriber owns a truck \\
rv & Subscriber owns a recreational vehicle \\
occprof & Occupation - professional \\
occcler & Occupation - clerical \\
occcrft & Occupation - crafts \\
occstud & Occupation - student \\
occhmkr & Occupation - homemaker \\
occret & Occupation - retired \\
occself & Occupation - self-employed \\
ownrent & Home ownership is missing \\
marryun & Marital status unknown \\
marryyes & Married \\
mailord & Buys via mail order \\
mailres & Responds to mail offers \\
mailflag & Has chosen not to be solicited by mail \\
travel & Has traveled to non-US country \\
pcown & Owns a personal computer \\
creditcd & Possesses a credit card \\
retdcalls & Number of calls previously made to retention team \\
retaccpt & Number of previous retention offers accepted \\
newcelly & Known to be a new cell phone user \\
newcelln & Known not to be a new cell phone user \\
refer & Number of referrals made by subscriber \\
incmiss & Income data is missing \\
income & Income (0=>missing) \\
mcycle & Owns a motorcycle \\
setprcm & Missing data on handset price \\
setprc & Handset price (0=>missing) \\
retcall & Customer has made call to retention team \\
\hline
\end{tabular}
\end{table}






\begin{table}[ht]
    \centering
    \caption{Comparison of performance metrics with adding top 1-5 highly associated fuzzy churn patterns for datasets 1-4.}
    \begin{tabular}{|c|l|c|c|c|c|c|c|c|c|}
    \hline
        \multicolumn{10}{|c|}{\textbf{Performance Metrics}} \\
    \hline
        \textbf{Dataset} & \textbf{Metrics} & \textbf{RF\cite{wu2021integrated}} & \textbf{XGBoost\cite{pamina2019effective}} & \textbf{1\textsuperscript{st}} & \textbf{2\textsuperscript{nd}} & \textbf{3\textsuperscript{rd}} & \textbf{4\textsuperscript{th}} & \textbf{5\textsuperscript{th}} & \textbf{AVG} \\
    \hline
        \multirow{5}{*}{1} & AUC & 91.3\% & 91.2\% & 91.2\% & \textbf{91.3\%} & \textbf{91.4\%} & \textbf{91.6\%} & \textbf{92.7\%} & \textbf{91.6\%} \\
         & Accuracy & 95.3\% & 95.7\% & \textbf{95.8\%} & \textbf{95.8\%} & \textbf{96.0\%} & \textbf{95.8\%} & 95.7\% & \textbf{95.8\%} \\
         & Recall & 71.9\% & 76.2\% & 76.2\% & 76.2\% & \textbf{79.2\%} & \textbf{77.2\%} & \textbf{77.2\%} & \textbf{77.2\%} \\
         & Precision & 91.7\% & 93.9\% & \textbf{95.1\%} & \textbf{95.1\%} & 93.0\% & 93.9\% & 92.8\% & \textbf{94.0\%} \\
         & F1 Score & 80.4\% & 84.2\% & \textbf{84.7\%} & \textbf{84.7\%} & \textbf{85.6\%} & \textbf{84.8\%} & \textbf{84.4\%} & \textbf{84.8\%} \\
    \hline
        \multirow{5}{*}{2} & AUC & 90.5\% & 90.6\% & 90.6\% & 90.6\% & 90.6\% & \textbf{91.0\%} & 90.5\% & \textbf{90.7\%}\\
        & Accuracy & 94.3\% & 95.6\% & 95.6\% & 95.6\% & \textbf{95.8\%} & 95.6\% & \textbf{95.8\%} & \textbf{95.7\%}\\
        & Recall & 81.5\% & 77.9\% & 77.9\% & \textbf{79.4\%} & \textbf{79.4\%} & \textbf{78.9\%} & \textbf{78.4\%} & \textbf{78.8\%} \\
        & Precision & 81.5\% & 92.1\% & 92.1\% & 90.6\% & 91.7\% & 91.1\% & \textbf{92.7\%} & 91.6\% \\
        & F1 Score & 81.5\% & 84.4\% & 84.4\% & \textbf{84.7\%} & \textbf{85.1\%} & \textbf{84.6\%} & \textbf{85.0\%} & \textbf{84.8\%} \\
    \hline
    \multirow{5}{*}{3} & AUC & 97.6\% & 98.5\% & \textbf{98.6\%} & 98.5\% & \textbf{98.7\%} & \textbf{98.6\%} & \textbf{98.6\%} & \textbf{98.6\%} \\
    & Accuracy & 94.3\% & 96.2\% & \textbf{96.7\%} & \textbf{96.5\%} & \textbf{96.7\%} & \textbf{96.7\%} & \textbf{96.7\%} & \textbf{96.7\%} \\
    & Recall & 85.5\% & 85.5\% & \textbf{86.7\%} & 85.5\% & \textbf{86.7\%} & 85.5\% & \textbf{86.7\%} & \textbf{86.2\%} \\
    & Precision & 82.5\% & 85.5\% & \textbf{87.8\%} & \textbf{87.6\%} & \textbf{87.8\%} & \textbf{88.7\%} & \textbf{87.8\%} & \textbf{87.9\%} \\
    & F1 Score & 83.9\% & 85.5\% & \textbf{87.2\%} & \textbf{86.5\%} & \textbf{87.2\%} & \textbf{87.1\%} & \textbf{87.2\%} & \textbf{87.0\%} \\
\hline
    \multirow{5}{*}{4} & AUC & 62.9\% & 65.3\% & \textbf{65.6\%} & \textbf{65.6\%} & 65.3\% & 65.3\% & \textbf{65.6\%} & \textbf{65.5\%} \\
    & Accuracy & 69.2\% & 63.6\% & \textbf{64.0\%} & \textbf{64.0\%} & \textbf{64.2\%} & \textbf{64.2\%} & \textbf{64.4\%} & \textbf{64.2\%} \\
    & Recall & 18.3\% & 52.6\% & \textbf{53.5\%} & \textbf{53.5\%} & \textbf{53.3\%} & \textbf{53.3\%} & \textbf{55.0\%} & \textbf{53.7\%} \\
    & Precision & 40.8\% & 39.2\% & \textbf{39.7\%} & \textbf{39.7\%} & \textbf{40.0\%} & \textbf{40.0\%} & \textbf{40.4\%} & \textbf{40.0\%} \\
    & F1 Score & 25.3\% & 44.9\% & \textbf{45.6\%} & \textbf{45.6\%} & \textbf{45.7\%} & \textbf{45.7\%} & \textbf{46.6\%} & \textbf{45.8\%} \\
\hline
    \end{tabular}
    \label{tab:datasets_performance_enhancement}
\end{table}
